RAGTruth: A Hallucination Corpus for Developing Trustworthy Retrieval-Augmented Language Models

Retrieval-augmented generation (RAG) has become a main technique for alleviating hallucinations in large language models (LLMs). Despite the integration of RAG, LLMs may still present unsupported or contradictory claims to the retrieved contents. In order to develop effective hallucination prevention strategies under RAG, it is important to create benchmark datasets that can measure the extent of hallucination. This paper presents RAGTruth, a corpus tailored for analyzing word-level hallucinations in various domains and tasks within the standard RAG frameworks for LLM applications. RAGTruth comprises nearly 18,000 naturally generated responses from diverse LLMs using RAG. These responses have undergone meticulous manual annotations at both the individual cases and word levels, incorporating evaluations of hallucination intensity. We not only benchmark hallucination frequencies across different LLMs, but also critically assess the effectiveness of several existing hallucination detection methodologies. Furthermore, we show that using a high-quality dataset such as RAGTruth, it is possible to finetune a relatively small LLM and achieve a competitive level of performance in hallucination detection when compared to the existing prompt-based approaches using state-of-the-art large language models such as GPT-4.

==> Tables/4-multilevel.tex <==
\begin{table}[!ht]
\renewcommand{\arraystretch}{1.5}

\small
\centering
    \begin{tabular}{lcc}
    \toprule
    % \multirow{2}{*}{Overall}  & \multicolumn{12}{c}{\textsc{Hallucination Detection}}\\
     & \multicolumn{1}{c}{\textsc{Easy}} & \multicolumn{1}{c}{\textsc{Difficult}} \\
     % \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    Overall \\
    QA \\
    Sum \\ 
    D2T \\



    \bottomrule
    \end{tabular}
    \caption{}
    \label{tab:3-statistic}
\end{table}


==> Tables/6-type-result.tex <==
% \begin{table*}[!ht]
% \scriptsize
% \centering
%     \begin{tabular}{l|cccccccccccc}
%     \toprule
%     \multirow{2}{*}{Methods}  & \multicolumn{3}{c}{\textsc{Subtle Conflict}} & \multicolumn{3}{c}{\textsc{Evident Conflict}} & \multicolumn{3}{c}{\textsc{Subtle Baseless Info}} & \multicolumn{3}{c}{\textsc{Evident Baseless Info}}  \\
%      \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13} 
%      & Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1\\
%      \midrule
%      Prompt$_\textrm{gpt-3.5-turbo}$ & 0 & 0 & 0 & 12.5 & 0.2 & 0.4 & 0 & 0 & 0 & 50.0 & 0.8 & 1.5\\
%      Prompt$_\textrm{gpt-4-turbo}$ & 0.2 & 30.0 & 0.3 & 7.6 & 54.6 & 13.3 & 2.6 & 42.5 & 4.8 & 13.9 & 52.3 & 21.9\\
%      Finetuned Llama-2-13B & 0.1 & 8.3 & 0.3 & 17.3 & 43.5 & 24.8 & 7.0 & 41.0 & 12.0 & 35.3 & 46.5 & 40.1  \\
%     \bottomrule
%     \end{tabular}
%     \caption{The span-level detection results of different models on four types of hallucinations. \textbf{Bold} denotes the best of each method. The footnote (if has) represents the base model we used to call in the baseline methods.}
%     \label{tab:6-type-result}
% \end{table*}


\begin{table*}[!ht]
\scriptsize
\centering
    \begin{tabular}{l|cccc}
    \toprule
    Methods  & \textsc{Subtle Conflict} & \textsc{Evident Conflict} & \textsc{Subtle Baseless Info} & \textsc{Evident Baseless Info}  \\

     \midrule
     Prompt$_\textrm{GPT-3.5-turbo}$  & 0   & 0.2  & 0  & 0.8 \\
     Prompt$_\textrm{GPT-4-turbo}$  & 30.0  & 54.6 & 42.5 & 52.3 \\
     Finetuned Llama-2-13B & 8.3 & 43.5 & 41.0 & 46.5  \\
    \bottomrule
    \end{tabular}
    \caption{The span-level recalls of different models on four types of hallucinations. The footnote (if has) represents the base model we used to call in the baseline methods. \red{replace this table with a figure}}
    \label{tab:6-type-result}
\end{table*}


==> Tables/due_to_null.tex <==
% \begin{table*}[t]
% % \small
% \centering
% \scriptsize
% % \scalebox{0.9}{
% \begin{tabular}{l|ccccccccc}
% \toprule
% \multirow{2}{*}{Task} & \multirow{2}{*}{\# Instance} & \multirow{2}{*}{\# Resp.} & \multicolumn{2}{c}{\textsc{Context Length}} & \multicolumn{2}{c}{\textsc{Resp. Length}} &\multicolumn{3}{c}{\textsc{Hallucination}} \\
% \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10}
%   & & & Mean  & Max  & Mean  & Max & \# Resp. & \% Resp. & \# Span \\
% \midrule
% Question Answering & 989 & 5934 & 243 & 509 & 119 &381 & 1724 & 29.1\% & 2927 \\
% Data-to-text Writing & 1033  & 6198 & 354 & 1253 & 159 & 369 & 4254 & 68.6\% & 9290 \\
% Summarization(CNN/DM) & 628 & 3768 & 648 & 1749 & 124 & 632 & 1165 & 30.9\% & 1474 \\
% Summarization(Recent News) & 315 & 1890 & 369 & 481  & 89  & 240  & 521 & 27.6\% & 598 \\
% \midrule
% Overall & 2965 & 17790 & 381 & 1749 & 131 & 632 & 7664 & 43.1\% & 14289 \\
% \bottomrule
% \end{tabular}
% % }
% \caption{The basic statistics of \CorpusName. Here "Resp." stands for "Response".}
% \label{tab:basic_stat}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\centering
\scriptsize
\begin{tabular}{ccccc}
\toprule
\textsc{Task}                                                                            & \textsc{Model}               & \textsc{\# Implicit True Span} & \textsc{\# Hallucination Span} & \textsc{Ratio} \\
\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Question\\ Answering\end{tabular}}   & GPT-3.5-turbo-0613  & 33                    & 89                    & 0.371 \\
                                                                                & GPT-4-0613          & 15                    & 51                    & 0.294 \\
                                                                                & Llama-2-7B-chat     & 251                   & 1010                  & 0.249 \\
                                                                                & Llama-2-13B-chat    & 215                   & 654                   & 0.329 \\
                                                                                & Llama-2-70B-chat    & 168                   & 529                   & 0.318 \\
                                                                                & Mistral-7B-Instruct & 164                   & 594                   & 0.276 \\
\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Data-to-text\\ Writing\end{tabular}} & GPT-3.5-turbo-0613  & 52                    & 384                   & 0.135 \\
                                                                                & GPT-4-0613          & 24                    & 354                   & 0.068 \\
                                                                                & Llama-2-7B-chat     & 195                   & 1775                  & 0.110 \\
                                                                                & Llama-2-13B-chat    & 260                   & 2803                  & 0.09  \\
                                                                                & Llama-2-70B-chat    & 274                   & 1834                  & 0.149 \\
                                                                                & Mistral-7B-Instruct & 102                   & 2140                  & 0.048 \\
\midrule
\multirow{6}{*}{Summarization}                                                  & GPT-3.5-turbo-0613  & 14                    & 60                    & 0.233 \\
                                                                                & GPT-4-0613          & 10                    & 80                    & 0.125 \\
                                                                                & Llama-2-7B-chat     & 44                    & 517                   & 0.085 \\
                                                                                & Llama-2-13B-chat    & 28                    & 342                   & 0.082 \\
                                                                                & Llama-2-70B-chat    & 27                    & 245                   & 0.110 \\
                                                                                & Mistral-7B-Instruct & 52                    & 828                   & 0.063 \\
\bottomrule
\end{tabular}
\caption{The majority of implicit truths appear in two types of tasks: question answering and data-to-text writing.}
\label{tab:implicit_true}
\end{table*}

==> Tables/resp_len_vs_halu.tex <==
\begin{table}[!t]
\scriptsize
\centering
    \begin{tabular}{l|ccccc}
    \toprule
    \multirow{2}{*}{Tasks} & \multicolumn{5}{c}{Response Length Bucket} \\
     &  1\# &  2\# &  3\# &  4\# &  5\# \\
     \midrule
     Summary  & 0.35   & 0.33  & 0.33 & 0.47 & 0.40 \\
     Data2text  & 1.22  & 1.19 & 1.60 & 1.82 & 1.64 \\
     QA & 0.34 & 0.27 & 0.38 & 0.66 & 1.24  \\
    \bottomrule
    \end{tabular}
    \caption{Average number of hallucinations per response length bucket for the three types of tasks.}
    \label{tab:rl-vs-halu}
\end{table}


==> Tables/statistic.tex <==
\begin{table*}[!ht]
\renewcommand{\arraystretch}{1.5}

\small
\centering
    \begin{tabular}{lc|cccccc}
    \toprule
    % \multirow{2}{*}{Overall}  & \multicolumn{12}{c}{\textsc{Hallucination Detection}}\\
     & & \multicolumn{3}{c}{\textsc{Response}} & \multicolumn{3}{c}{\textsc{Span}} \\
     \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    \multirow{2}{*}{Overall} & \# Training Examples & \multicolumn{6}{c} {10000} \\
     & \# Test Examples & \multicolumn{6}{c} {2000} \\

     \midrule
     \multirow{3}{*}{Question Answering} & \# Examples \\
      & Avg. Length \\
      & Model Distribution & 20\% &  20\%& 20\%& 20\%& 20\%& 20\% \\

     \midrule
     \multirow{3}{*}{Summarization} & \# Examples \\
      & Avg. Length \\
      & Model Distribution & 20\% &  20\%& 20\%& 20\%& 20\%& 20\% \\
         \midrule
     \multirow{3}{*}{Data2Text} & \# Examples \\
      & Avg. Length \\
      & Model Distribution & 20\% &  20\%& 20\%& 20\%& 20\%& 20\% \\

    \bottomrule
    \end{tabular}
    \caption{Overall detection performance for each baseline methods across different tasks. (\textsc{Sum}) means we only test on the summarization task of HaluEval benchmark.}
    \label{tab:3-statistic}
\end{table*}

